A ProbLog program to infer individual genotypes from familial phenotypes in autosomal, X-linked, and Y-linked Mendelian disorders

The automated reconstruction of patient family history is a common challenge in genetic counseling for disease prevention. Such a family history is usually determined for a particular subset of diseases that are Mendelian, i.e. monogenic, and classified into three categories depending on the chromosome the gene is located: autosomal, X-linked or Y-linked. Mendel's inheritance laws allow for simple probabilistic modeling of the genetic transmission of monogenic disorders. Genetic counsellors use knowledge about the patient's family history and Mendelian laws for assessing risks of transmitting or inheriting congenital conditions. We present mendelprob.pl, a probabilistic logic programming algorithm in ProbLog for deriving probabilities of inheritance of genotypes and phenotypes for genes with two alleles through multiple generations. In particular, the user can input genotypes and phenotypes for a patient and its family, and automatically determine the most probable genetic family history. We illustrate the ProbLog model on practical examples of patient pedigrees from the literature and from a genetic counseling handbook. We show that our method correctly infers probability of individual genotypes from knowledge about familial genotypes, yielding the same results as tool pedprobr. However, unlike pedprobr, our approach can exploit knowledge about familial phenotypes. It can also directly distinguish between autosomal, X-linked, and Y-linked disorders, using its intuitive logical modelling. We provide our ProbLog tool for free and open-source on GitHub, making it easily available for genetic counsellors. We conclude on the importance of providing explainable formal methods for a task that clinicians might want to perform using proprietary software.

==> eptcsdata.tex <==
\providecommand{\firstpage}{465}
\providecommand{\publicationstatus}{W. Faber, L. Giordano, R. Rocha, V. Santos Costa (Eds.):\\ 42nd International Conference on Logic Programming (ICLP 2026)\\
EPTCS 450, 2026, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{http://dx.doi.org/10.4204/EPTCS.450.34}{10.4204/EPTCS.450.34}}

